Zero-shot Referring Image Segmentation with Global-Local Context Features

Referring image segmentation (RIS) aims to find a segmentation mask given a referring expression grounded to a region of the input image. Collecting labelled datasets for this task, however, is notoriously costly and labor-intensive. To overcome this issue, we propose a simple yet effective zero-shot referring image segmentation method by leveraging the pre-trained cross-modal knowledge from CLIP. In order to obtain segmentation masks grounded to the input text, we propose a mask-guided visual encoder that captures global and local contextual information of an input image. By utilizing instance masks obtained from off-the-shelf mask proposal techniques, our method is able to segment fine-detailed Istance-level groundings. We also introduce a global-local text encoder where the global feature captures complex sentence-level semantics of the entire input expression while the local feature focuses on the target noun phrase extracted by a dependency parser. In our experiments, the proposed method outperforms several zero-shot baselines of the task and even the weakly supervised referring expression segmentation method with substantial margins. Our code is available at https://github.com/Seonghoon-Yu/Zero-shot-RIS.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> rebuttal/Quantitative.tex <==

\setlength{\columnsep}{8pt}%
\begin{wraptable}{r}{0.6\linewidth}
\vspace{-0.5cm}
\caption{\footnotesize{Mask-class accuracy and class-conditioned oIoU with different feature types on RefCOCOg.}}
\vspace{-0.3cm}
\centering
% \tiny
% \scriptsize
% \setlength{\columnsep}{0pt}%
\scalebox{0.7}{
\begin{tabular}{l|ccc}
\hline
Feature type & {MC-ACC}   & {CC-oIoU} & {oIoU}  \\ \hline
Global                                                                    & 78.90 & 33.10    & 27.03 \\
Local                                                                     & 83.36 & 29.94    & 25.23 \\
Global-Local                                                              & 84.32 & 35.61    & 31.11 \\ \hline
\end{tabular}
}
% \vspace{-0.3cm}



% \scalebox{0.6}{
% \begin{tabular}{l|ccccccccc}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ features\end{tabular}} & \multicolumn{9}{c}{Textual features}                                                                                             \\ \cline{2-10} 
%                                                                           & \multicolumn{3}{c|}{Global}                   & \multicolumn{3}{c|}{Local}                    & \multicolumn{3}{c}{Global-Local} \\ \cline{2-10} 
%                                                                           & Acc   & cc\_oIoU & \multicolumn{1}{l|}{oIoU}  & Acc   & cc\_oIoU & \multicolumn{1}{l|}{oIoU}  & Acc      & cc\_oIoU    & oIoU    \\ \hline
% Global                                                                     & 78.90 & 33.10    & \multicolumn{1}{l|}{27.03} & 81.82 & 32.05    & \multicolumn{1}{l|}{27.37} & 80.94    & 32.90       & 27.60   \\ \hdashline[1pt/1pt]
% Local                                                                      & 81.43 & 34.35    & \multicolumn{1}{l|}{28.69} & 83.36 & 29.94    & \multicolumn{1}{l|}{25.23} & 84.67    & 33.93       & 29.48   \\ \hdashline[1pt/1pt]
% G-L                                                                        & 81.90 & 35.84    & \multicolumn{1}{l|}{30.18} & 82.63 & 32.52    & \multicolumn{1}{l|}{27.94} & 84.32    & 35.61       & 31.11   \\ \hline
% \end{tabular}
% }







% \scalebox{0.8}{
% \begin{tabular}{l|cc|cc|cc}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ features\end{tabular}} & \multicolumn{6}{c}{Textual features}                                                                                                                                                                                                          \\ \cline{2-7} 
%                                                                           & \multicolumn{2}{c|}{Global}                                                          & \multicolumn{2}{c|}{Local}                                                           & \multicolumn{2}{c}{Global-Local}                                \\ \cline{2-7} 
%                                                                           & Acc   & oIoU  & Acc   & oIoU  & Acc  & oIoU  \\ \hline
% Global                                                                     & 78.90 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}33.10\\ 27.03$\dag$ \end{tabular}} & 81.82 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}32.05\\ 27.37$\dag$ \end{tabular}} & 80.94 & \begin{tabular}[c]{@{}c@{}}32.90\\ 27.60$\dag$\end{tabular} \\ \hdashline[1pt/1pt]
% Local                                                                      & 81.43 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}34.35\\ 28.69$\dag$ \end{tabular}} & 83.36 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}29.94\\ 25.23$\dag$ \end{tabular}} & 84.67 & \begin{tabular}[c]{@{}c@{}}33.93\\ 29.48$\dag$ \end{tabular} \\ \hdashline[1pt/1pt]
% G-L                                                                        & 81.90 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}35.84\\ 30.18$\dag$ \end{tabular}} & 82.63 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}32.52\\ 27.94$\dag$ \end{tabular}} & 84.32 & \begin{tabular}[c]{@{}c@{}}35.61\\ 31.11$\dag$ \end{tabular} \\ \hline
% \end{tabular}
% }


% \begin{tabular}{l|cc|cc|cc}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ features\end{tabular}} & \multicolumn{6}{c}{Textual features}                                                                                                                                                                                                          \\ \cline{2-7} 
%                                                                           & \multicolumn{2}{c|}{Global}                                                          & \multicolumn{2}{c|}{Local}                                                           & \multicolumn{2}{c}{Global-Local}                                \\ \cline{2-7} 
%                                                                           & Acc   & oIoU  & Acc   & oIoU  & Acc  & oIoU  \\ \hline
% Global                                                                     & 78.90 & \multicolumn{1}{c;{1pt/1pt}}{\begin{tabular}[c]{@{}c@{}}33.10\\ 27.03$\dag$ \end{tabular}} & 81.82 & \multicolumn{1}{c;{1pt/1pt}}{\begin{tabular}[c]{@{}c@{}}32.05\\ 27.37$\dag$ \end{tabular}} & 80.94 & \begin{tabular}[c]{@{}c@{}}32.90\\ 27.60$\dag$\end{tabular} \\ \hdashline[1pt/1pt]
% Local                                                                      & 81.43 & \multicolumn{1}{c;{1pt/1pt}}{\begin{tabular}[c]{@{}c@{}}34.35\\ 28.69$\dag$ \end{tabular}} & 83.36 & \multicolumn{1}{c;{1pt/1pt}}{\begin{tabular}[c]{@{}c@{}}29.94\\ 25.23$\dag$ \end{tabular}} & 84.67 & \begin{tabular}[c]{@{}c@{}}33.93\\ 29.48$\dag$ \end{tabular} \\ \hdashline[1pt/1pt]
% G-L                                                                        & 81.90 & \multicolumn{1}{c;{1pt/1pt}}{\begin{tabular}[c]{@{}c@{}}35.84\\ 30.18$\dag$ \end{tabular}} & 82.63 & \multicolumn{1}{c;{1pt/1pt}}{\begin{tabular}[c]{@{}c@{}}32.52\\ 27.94$\dag$ \end{tabular}} & 84.32 & \begin{tabular}[c]{@{}c@{}}35.61\\ 31.11$\dag$ \end{tabular} \\ \hline
% \end{tabular}


% \begin{tabular}{l|cccccc}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ features\end{tabular}} & \multicolumn{6}{c}{Textual features}                                                                                                                                                                                                          \\ \cline{2-7} 
%                                                                           & \multicolumn{2}{c|}{Global}                                                          & \multicolumn{2}{c|}{Local}                                                           & \multicolumn{2}{c}{Global-Local}                                \\ \cline{2-7} 
%                                                                           & Acc   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}oIoU\\ (Final)\end{tabular}}  & Acc   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}oIoU\\ (Final)\end{tabular}}  & Acc  & \begin{tabular}[c]{@{}c@{}}oIoU\\ (Final)\end{tabular}  \\ \hline
% Global                                                                     & 78.90 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}33.10\\ (27.03)\end{tabular}} & 81.82 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}32.05\\ (27.37)\end{tabular}} & 80.94 & \begin{tabular}[c]{@{}c@{}}32.90\\ (27.60)\end{tabular} \\ \hdashline[1pt/1pt]
% Local                                                                      & 81.43 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}34.35\\ (28.69)\end{tabular}} & 83.36 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}29.94\\ (25.23)\end{tabular}} & 84.67 & \begin{tabular}[c]{@{}c@{}}33.93\\ (29.48)\end{tabular} \\ \hdashline[1pt/1pt]
% G-L                                                                        & 81.90 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}35.84\\ (30.18)\end{tabular}} & 82.63 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}32.52\\ (27.94)\end{tabular}} & 84.32 & \begin{tabular}[c]{@{}c@{}}35.61\\ (31.11)\end{tabular} \\ \hline
% \end{tabular}

% \begin{tabular}{l|cllcllcll}
% \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Visual\\ features\end{tabular}}} & \multicolumn{9}{c}{Textual features}                                                                                                                       \\ \cline{2-10} 
% \multicolumn{1}{c|}{}                                                                           & \multicolumn{3}{c|}{Global}                            & \multicolumn{3}{c|}{Local}                             & \multicolumn{3}{c}{Global-Local}         \\ \cline{2-10} 
% \multicolumn{1}{c|}{}                                                                           & \multicolumn{2}{c}{Acc}   & \multicolumn{1}{l|}{oIoU}  & \multicolumn{2}{c}{Acc}   & \multicolumn{1}{l|}{oIoU}  & \multicolumn{2}{c}{Acc}   & oIoU         \\ \hline
% \multirow{2}{*}{G}                                                                              & \multicolumn{2}{c}{12.34} & \multicolumn{1}{l|}{12.44} & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{12.22} & \multicolumn{2}{c}{11.24} & 21.33        \\ \cline{2-10} 
%                                                                                                 & \multicolumn{3}{l|}{12.44(Final)}                      & \multicolumn{3}{l|}{12.24(Final)}                      & \multicolumn{3}{l}{23.44(Final)}         \\ \hline
% \multirow{2}{*}{L}                                                                              & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{23.12} & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{21.33} & \multicolumn{2}{c}{11.23} & 12.33        \\ \cline{2-10} 
%                                                                                                 & \multicolumn{3}{l|}{21.43(Final)}                      & \multicolumn{3}{l|}{21.42(Final}                       & \multicolumn{3}{l}{12.34(FInal)}         \\ \hline
% \multirow{2}{*}{G-L}                                                                            & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{12.33} & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{12.33} & \multicolumn{2}{c}{11.23} & 12.34        \\ \cline{2-10} 
%                                                                                                 & \multicolumn{3}{l|}{12.24(FInal)}                      & \multicolumn{3}{l|}{21.42(Final}                       & \multicolumn{3}{l}{12.42(Final)}         \\ \cline{1-1}
% \end{tabular}

% \begin{tabular}{lcllcllcll}
% \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Visual\\ features\end{tabular}}} & \multicolumn{9}{c}{Textual features}                                                                                                                       \\ \cline{2-10} 
% \multicolumn{1}{c|}{}                                                                           & \multicolumn{3}{c|}{Global}                            & \multicolumn{3}{c|}{Local}                             & \multicolumn{3}{c}{Global-Local}         \\ \cline{2-10} 
% \multicolumn{1}{c|}{}                                                                           & \multicolumn{2}{c}{Acc}   & \multicolumn{1}{l|}{oIoU}  & \multicolumn{2}{c}{Acc}   & \multicolumn{1}{l|}{oIoU}  & \multicolumn{2}{c|}{Acc}  & oIoU         \\ \hline
% \multicolumn{1}{l|}{\multirow{2}{*}{G}}                                                         & \multicolumn{2}{c}{12.34} & \multicolumn{1}{l|}{12.44} & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{12.22} & \multicolumn{2}{c}{11.24} & 21.33        \\
% \multicolumn{1}{l|}{}                                                                           & \multicolumn{3}{l}{12.44(Final)}                       & \multicolumn{3}{l}{12.24(Final)}                       & \multicolumn{3}{l}{23.44(Final)}         \\
% \multicolumn{1}{l|}{\multirow{2}{*}{L}}                                                         & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{23.12} & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{21.33} & \multicolumn{2}{c}{11.23} & 12.33        \\
% \multicolumn{1}{l|}{}                                                                           & \multicolumn{3}{l}{21.43(Final)}                       & \multicolumn{3}{l}{21.42(Final}                        & \multicolumn{3}{l}{12.34(FInal)}         \\
% \multicolumn{1}{l|}{\multirow{2}{*}{G-L}}                                                       & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{12.33} & \multicolumn{2}{c}{11.23} & \multicolumn{1}{l|}{12.33} & \multicolumn{2}{c}{11.23} & 12.34        \\ \cline{2-10} 
% \multicolumn{1}{l|}{}                                                                           & \multicolumn{3}{l}{}                                   & \multicolumn{3}{l}{}                                   & \multicolumn{3}{l}{}                     \\ \cline{1-1}
% \end{tabular}





% \begin{tabularx}{\columnwidth}{l|cllcllcll}
% \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Visual\end{tabular}}} & \multicolumn{9}{c}{Textual features}                                                                                                                                         \\ \cline{2-10} 
% \multicolumn{1}{c|}{}                                                                           & \multicolumn{3}{c|}{Global}                                  & \multicolumn{3}{c|}{Local}                                   & \multicolumn{3}{c}{Global-Local}               \\ \cline{2-10} 
% \multicolumn{1}{c|}{}                                                                           & \multicolumn{2}{c}{Acc / oIoU}  & \multicolumn{1}{l|}{Final} & \multicolumn{2}{c}{Acc / oIoU}  & \multicolumn{1}{l|}{Final} & \multicolumn{2}{c|}{Acc / oIoU} & Final        \\ \hline
% G                                                                                               & \multicolumn{2}{c}{1234 / 1234} & \multicolumn{1}{l|}{1244}  & \multicolumn{2}{c}{1124 / 1234} & \multicolumn{1}{l|}{1244}  & \multicolumn{2}{c}{1124 / 1234} & 2133         \\
% L                                                                                               & \multicolumn{2}{c}{1123 / 1234} & \multicolumn{1}{l|}{2312}  & \multicolumn{2}{c}{1123 / 1234} & \multicolumn{1}{l|}{2133}  & \multicolumn{2}{c}{1123 / 1234} & 1233         \\
% G-L                                                                                             & \multicolumn{2}{c}{1123 / 1234} & \multicolumn{1}{l|}{1233}  & \multicolumn{2}{c}{1123 / 1234} & \multicolumn{1}{l|}{1233}  & \multicolumn{2}{c}{1123 / 1234} & 1234         \\ \hline
% \end{tabularx}



% \begin{tabular}{l|cccccc}
% \multicolumn{1}{c|}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Visual\\ features\end{tabular}}} & \multicolumn{6}{c}{Textual features}                                                                                                           \\ \cline{2-7} 
% \multicolumn{1}{c|}{}                                                                           & \multicolumn{2}{c|}{Global}                          & \multicolumn{2}{c|}{Local}                           & \multicolumn{2}{c}{Global-Local} \\ \cline{2-7} 
% \multicolumn{1}{c|}{}                                                                           & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{oIoU} & \multicolumn{1}{c|}{Acc} & \multicolumn{1}{c|}{oIoU} & \multicolumn{1}{c|}{Acc}  & oIoU \\ \hline
% Global                                                                                          & \multicolumn{1}{c|}{1}   & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{1}   & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{1}    & 1    \\
% Local                                                                                           & \multicolumn{1}{c|}{1}   & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{1}   & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{1}    & 1    \\
% Global-Local                                                                                    & \multicolumn{1}{c|}{1}   & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{1}   & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{1}    & 1    \\ \hline
% \end{tabular}


% \begin{tabular}{l|l|c|c|c}
% \hline
% \multicolumn{2}{c|}{\multirowcell{2.2}{Encoder Variants}}  &   \multicolumn{3}{c}{Textual features} \\
% \cline{3-5}
%  \multicolumn{2}{c|}{} & \makecell{Global\\Accuracy / oIoU}         & Local         & Global-Local  \\ \hline
% \multirow{3}{*}{\makecell{ Visual \\ features }}& Global        &  78.90 / 33.10             &  81.82 / 32.05   &     80.94 / 32.90\\
% & Local         &  81.43 / 34.35    &   83.36 / 29.94           &     84.67 / 33.93         \\
% & Global-Local        &  81.90 / 35.84             &  82.63 / 32.52            &     84.32 / 35.61 \\
% \hline
% \end{tabular}


% \begin{tabular}{l|l|c|c|c}
% \hline
% \multicolumn{2}{c|}{\multirowcell{2.2}{Encoder Variants}}  &   \multicolumn{3}{c}{Textual features} \\
% \cline{3-5}
%  \multicolumn{2}{c|}{} & Global         & Local         & Global-Local  \\ \hline
% \multirow{3}{*}{\makecell{ Visual \\ features }}& Global        &  78.90 / 33.10             &  81.82 / 32.05   &     80.94 / 32.90\\
% & Local         &  81.43 / 34.35    &   83.36 / 29.94           &     84.67 / 33.93         \\
% & Global-Local        &  81.90 / 35.84             &  82.63 / 32.52            &     84.32 / 35.61 \\
% \hline
% \end{tabular}

% \begin{tabular}{l|l|ccc}
% \hline
% \multicolumn{2}{c|}{\multirowcell{2.2}{Encoder Variants}}  &   \multicolumn{3}{c}{Textual features} \\
% \cline{3-5}
%  \multicolumn{2}{c|}{} & Global         & Local         & Global-Local  \\ \hline
% \multirow{3}{*}{\makecell{ Visual \\ features }}& Global        &  27.03             &  {27.37}   &     \underline{27.60}\\
% & Local         &  {28.69}    &  25.23            &     \underline{29.48}         \\
% & Global-Local        &  \underline{30.18}             &  \underline{27.94}            &     \textbf{31.11} \\
% \hline
% \end{tabular}

% \begin{tabular}{l|l|c|c|c}
% \hline
% \multicolumn{3}{c|}{\multirowcell{2.2}{Encoder Variants}}  &   \multicolumn{3}{c}{Textual features} \\
% \cline{3-5}
%  \multicolumn{2}{c|}{} & Global         & Local         & Global-Local  \\ \hline
% \multirow{3}{*}{\makecell{ Visual \\ features }}& Global        &  78.90 / 33.10             &  81.82 / 32.05   &     80.94 / 32.90\\
% & Local         &  81.43 / 34.35    &   83.36 / 29.94           &     84.67 / 33.93         \\
% & Global-Local        &  81.90 / 35.84             &  82.63 / 32.52            &     84.32 / 35.61 \\
% \hline
% \end{tabular}
\label{tab:reburral:quantitative}
\vspace{-0.4cm}
\end{wraptable}

==> rebuttal/Zero-shot.tex <==
\begin{table}[H]
\centering
% \footnotesize
\vspace{-0.1cm}
\caption{Comparisons to supervised methods in zero-shot evaluation.
%$\dag$ denotes our re-implementation, since official pre-trained weigths are not released.
}
\label{tab:rebuttal:zero-shot}
\scalebox{0.7}{
\begin{tabular}{c|c|c|c}
\hline
% \multirow{2}{*}{Method} & \multirow{2}{*}{Train set} & \multicolumn{2}{c}{oIoU on PhraseCut val} \\ \cline{3-4} 
%                          &                            & {All}                    & {Unseen}                  \\ 
&&\multicolumn{2}{c}{oIoU on PhraseCut} \\\cline{3-4} 
Method & Train dataset & All & Unseen \\
                         \hline
\multirow{3}{*}{LAVT [49]}    & RefCOCO                    & 18.18                   & 15.26                  \\
                         & RefCOCO+                   & 17.50                   & 14.72                  \\
                         & RefCOCOg                   & 18.70                   & 15.49                  \\ \hdashline[1pt/1pt]
\multirow{3}{*}{CRIS [46]} & RefCOCO & 18.57 & 15.76 \\
                        & RefCOCO+ & 18.18 & 15.38 \\
                        & RefCOCOg & 19.68 & 16.22 \\ \hdashline[1pt/1pt]
%  \hline Ours(ResNet)             & N/A                  & 20.74                   & 19.56                  \\
Ours                & N/A                  & \textbf{22.91}                   & \textbf{21.80}                  \\ \hline
\end{tabular}
}



% \begin{tabular}{l|c|c|c}
% \hline
% \multirow{2}{*}{Method} & \multirow{2}{*}{Train set} & \multicolumn{2}{c}{PhraseCut val} \\ \cline{3-4} 
%                          &                            & oIoU                    & \makecell{unseen \\oIoU}                   \\ \hline
% \multirow{3}{*}{LAVT~\cite{lavt}}    & RefCOCO                    & 18.18                   & 15.26                  \\
%                          & RefCOCO+                   & 17.50                   & 14.72                  \\
%                          & RefCOCOg                   & 18.70                   & 15.49                  \\ \hdashline[1pt/1pt]
% \multirow{3}{*}{CRIS~\cite{cris} $\dag$} & RefCOCO & & \\
%                         & RefCOCO+ & & \\
%                         & RefCOCOg & & \\


% \hdashline[1pt/1pt]
% %  \hline Ours(ResNet)             & N/A                  & 20.74                   & 19.56                  \\
% Ours                & N/A                  & \textbf{22.91}                   & \textbf{21.80}                  \\ \hline
% \end{tabular}

\end{table}

% \begin{tabular}{l|l|cc}
% \hline
% \multirow{2}{*}{Methods} & \multirow{2}{*}{Train set} & \multicolumn{2}{c}{PhraseCut} \\ \cline{3-4} 
%                          &                            & oIoU                    & mIoU                   \\ \hline
% \multirow{3}{*}{LAVT}    & RefCOCO                    & 15.26                   & 16.83                  \\
%                          & RefCOCO+                   & 14.72                   & 16.81                  \\
%                          & RefCOCOg                   & 15.49                   & 15.53                  \\ \hline
% ours(ResNet)             & Zero-Shot                  & 19.56                   & 20.43                  \\
% ours(ViT)                & Zero-Shot                  & 21.80                   & 21.17                  \\ \hline
% \end{tabular}



==> tables/Total_Comparision.tex <==
\begin{table*}
\small
\centering
    \caption{Comparison with Zero-shot RIS baseline methods on three standard benchmark datasets. U: The UMD partition. G: The Google partition. All baseline methods use FreeSOLO as the mask proposal network. $\dag$ denotes the ImageNet pre-trained model. FreeSOLO upper bound means that the mIoU is computed between the GT mask and the maximum overlapped FreeSOLO mask with the GT mask.}
    % max overall IoU Mask of FreeSOLO outputs and GT mask 


\begin{tabular}{ll|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Methods}     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ Encoder\end{tabular}} & \multicolumn{3}{c|}{RefCOCO}                     & \multicolumn{3}{c|}{RefCOCO+}                    & \multicolumn{3}{c}{RefCOCOg}                     \\ \cline{3-11} 
                             &                                                                           & val            & test A         & test B         & val            & test A         & test B         & val            & test(U)        & val(G)         \\ \hline
\textbf{Zero-Shot Baselines} &                                                                           &                &                &                &                &                &                &                &                &                \\
CLIP Grad-CAM~\cite{}                     & ResNet-50                                                                 & 14.02          & 15.07          & 13.49          & 14.46          & 14.97          & 14.04          & 12.51          & 12.81          & 12.86          \\
MaskCLIP~\cite{}                     & ResNet-50                                                                 & 19.87          & 19.31          & 20.22          & 20.37          & 19.65          & 20.75          & 18.88          & 19.16          & 19.15          \\
Adapting CLIP~\cite{}                & ViT-B/32                                                                  & 21.71          & 20.31          & 22.63          & 22.61          & 20.91          & 23.46          & 25.52          & 25.38          & 25.29          \\
Crop method~\cite{}                  & ResNet-50                                                                 & 22.36          & 20.49          & 22.69          & 23.95          & 22.03          & 23.49          & 28.20          & 27.64          & 27.47          \\
Crop method~\cite{}                  & ViT-B/32                                                                  & 22.73          & 21.11          & 23.08          & 24.09          & 22.42          & 23.93          & 28.69          & 27.51          & 27.70          \\ \hline
Global-Local CLIP (ours)                         & ResNet-50                                                                 & 24.56          & 23.38          & 24.35          & 25.87          & 24.61          & 25.61          & 30.07          & 29.83          & 29.45          \\
Global-Local CLIP (ours)                         & ViT-B/32                                                                  & \textbf{24.88} & \textbf{23.61} & \textbf{24.66} & \textbf{26.16} & \textbf{24.90} & \textbf{25.83} & \textbf{31.11} & \textbf{30.96} & \textbf{30.69} \\ 
\hdashline[1pt/1pt]
FreeSOLO upper bound         & \multicolumn{1}{c|}{-}                                                    & 42.08          & 42.52          & 43.52          & 42.17          & 42.52          & 43.80          & 48.81          & 48.96          & 48.49          \\ \hline
\textbf{Weakly-supervised method} &                                                                           &                &                &                &                &                &                &                &                &                \\
TSEG~\cite{}     & ViT-S/16$^\dagger$                                                                  & 25.95          & -              & -              & 22.62          & -              & -              & 23.41          & -              & -              \\ \hline
\end{tabular}


% \begin{tabular}{l|l|ccc|ccc|ccc}
% \hline 
% \multirow{2}{*}{Methods} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Visual\\ Encoder\end{tabular}}} & \multicolumn{3}{c|}{Refcoco}                                               & \multicolumn{3}{c|}{Refcoco+}                                              & \multicolumn{3}{c}{Refcocog}                                                \\ \cline{3-11} 
% \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}                                                                          & \multicolumn{1}{c|}{val}            & \multicolumn{1}{c|}{test A} & test B & \multicolumn{1}{c|}{val}            & \multicolumn{1}{c|}{test A} & test B & \multicolumn{1}{c|}{val}            & \multicolumn{1}{c|}{test(U)} & val(G) \\ \hline
% Weakly-supervised method~\cite{}                     & \multicolumn{1}{c|}{ViT-S/16$^\dagger$}                                                                  & \multicolumn{1}{c|}{25.95}          & \multicolumn{1}{c|}{-}      & -      & \multicolumn{1}{c|}{22.62}          & \multicolumn{1}{c|}{-}      & -      & \multicolumn{1}{c|}{23.41}          & \multicolumn{1}{c|}{-}       & -      \\ \hline
% CLIP Grad-CAM                                      & ResNet-50                                                                                      & \multicolumn{1}{c|}{14.02}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{14.46}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{12.51}          & \multicolumn{1}{c|}{}        &        \\
% MaskCLIP                                      & ResNet-50                                                                                      & \multicolumn{1}{c|}{19.79}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{20.23}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{18.82}          & \multicolumn{1}{c|}{}        &        \\
% Adapting CLIP                                 & ViT-B/32                                                                                       & \multicolumn{1}{c|}{21.71}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{22.61}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{25.52}          & \multicolumn{1}{c|}{}        &        \\
% Crop method                                   & ResNet-50                                                                                      & \multicolumn{1}{c|}{22.36}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{23.95}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{28.20}          & \multicolumn{1}{c|}{}        &        \\
% Crop method                                   & ViT-B/32                                                                                       & \multicolumn{1}{c|}{22.73}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{24.09}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{28.69}          & \multicolumn{1}{c|}{}        &        \\ \hline
% Ours(Only visual)                             & ResNet-50                                                                                      & \multicolumn{1}{c|}{24.43}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{25.80}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{29.07}          & \multicolumn{1}{c|}{}        &        \\
% Ours(+ Global-Local text)                           & ResNet-50                                                                                      & \multicolumn{1}{c|}{24.56}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{25.87}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{30.07}          & \multicolumn{1}{c|}{}        &        \\
% Ours(Only visual)                             & ViT-B/32                                                                                       & \multicolumn{1}{c|}{24.85}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{26.14}          & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{30.18}          & \multicolumn{1}{c|}{}        &        \\
% Ours(+ Global-Local text)                           & ViT-B/32                                                                                       & \multicolumn{1}{c|}{\textbf{24.88}} & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{\textbf{26.16}} & \multicolumn{1}{c|}{}       &        & \multicolumn{1}{c|}{\textbf{31.11}} & \multicolumn{1}{c|}{}        &        \\ \hline
% FreeSOLO upper bound                          & \multicolumn{1}{c|}{-}                                                                         & \multicolumn{1}{c|}{42.08}          & \multicolumn{1}{c|}{42.52}  & 43.52  & \multicolumn{1}{c|}{42.17}          & \multicolumn{1}{c|}{42.52}  & 43.80  & \multicolumn{1}{c|}{48.81}          & \multicolumn{1}{c|}{48.96}   & 48.49  \\
% \hline
% \end{tabular}
  \label{tab:CoLoctable}

\end{table*}

==> tables/Total_Comparision_mIoU.tex <==
\begin{table*}[ht!]
\small
\centering
    \caption{Comparison with Zero-shot RIS baseline methods on three standard benchmark datasets. U: The UMD partition. G: The Google partition. All baseline methods use FreeSOLO as the mask proposal network. $\dag$ denotes the ImageNet pre-trained model. FreeSOLO upper bound means that the mIoU is computed between the GT mask and the maximum overlapped FreeSOLO mask with the GT mask.}
    % max overall IoU Mask of FreeSOLO outputs and GT mask 


\begin{tabular}{ll|ccc|ccc|ccc}
\hline
\multirow{2}{*}{Methods}            & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ Encoder\end{tabular}} & \multicolumn{3}{c|}{RefCOCO}                     & \multicolumn{3}{c|}{RefCOCO+}                    & \multicolumn{3}{c}{RefCOCOg}                     \\ \cline{3-11} 
                                    &                                                                           & val            & test A         & test B         & val            & test A         & test B         & val            & test(U)        & val(G)         \\ \hline
\textbf{Zero-Shot Baselines}        &                                                                           &                &                &                &                &                &                &                &                &                \\
Grad-CAM~\cite{}                    & ResNet-50                                                                 & 14.22          & 15.93          & 13.18          & 14.80         & 15.87          & 13.78        & 12.47          & 13.16          & 13.30          \\
MaskCLIP~\cite{}                    & ResNet-50                                                                 & 21.32          & 20.96          & 21.57          & 21.61          & 21.17          & 22.30          & 20.07          & 20.43          & 20.63          \\
Adapting CLIP~\cite{}               & ViT-B/32                                                                  & 23.43          & 22.07          & 24.62          & 24.51          & 22.64          & 25.37          & 27.57          & 27.34          & 27.69          \\
Cropping~\cite{}                 & ResNet-50                                                                 & 24.31          & 22.37          & 24.66          & 26.31          & 23.94          & 25.69          & 31.27          & 30.87          & 30.78          \\
Cropping~\cite{}                 & ViT-B/32                                                                  & 24.83          & 22.58          & 25.72          & 26.33          & 24.06          & 26.46          & 31.88          & 30.94          & 31.06          \\ \hline
Global-Local CLIP (ours)            & ResNet-50                                                                 & \textbf{26.70} & \textbf{24.99} & 26.48          & \textbf{28.22} & \textbf{26.54} & \textbf{27.86} & 33.02          & 33.12          & 32.79          \\
Global-Local CLIP (ours)            & ViT-B/32                                                                  & 26.20          & 24.94          & \textbf{26.56} & 27.80          & 25.64          & 27.84          & \textbf{33.52} & \textbf{33.67} & \textbf{33.61} \\ 
\hdashline[1pt/1pt]
FreeSOLO upper bound                & \multicolumn{1}{c|}{-}                                                    & 48.25          & 46.62          & 50.43          & 48.28          & 46.62          & 50.62          & 52.44          & 52.91          & 52.76          \\ \hline
\textbf{Weakly-supervised method}   &                                                                           &                &                &                &                &                &                &                &                &                \\
TSEG~\cite{}                        & ViT-S/16$^\dagger$                                                        & 25.95          & -              & -              & 22.62          & -              & -              & 23.41          & -              & -              \\ \hline
\end{tabular}
\label{tab:CoLoctable}

\end{table*}

==> tables/ViT_Token_masking_ablation.tex <==
% \begin{table*}
% \small
% \centering
% \caption{Token masking ablation in ViT, ViT-B/32, ViT-B/16, ViT-L/14 have 12, 12, 24 layers}
% \begin{tabular}{lccccccccc}
%                           & \multicolumn{3}{c}{RefCOCO(val)}                                                            & \multicolumn{3}{c}{RefCOCO+(val)}                                                              & \multicolumn{3}{c}{RefCOCOg(val)}                                                          \\ \hline
% \multicolumn{1}{l|}{Layer} & \multicolumn{1}{l}{ViT-B/32} & \multicolumn{1}{l}{ViT-B/16} & \multicolumn{1}{l|}{ViT-L/14} & \multicolumn{1}{l}{ViT-B/32} & \multicolumn{1}{l}{ViT-B/16} & \multicolumn{1}{l|}{ViT-L/14}    & \multicolumn{1}{l}{ViT-B/32} & \multicolumn{1}{l}{ViT-B/16} & \multicolumn{1}{l}{ViT-L/14} \\ \hline
% \multicolumn{1}{l|}{-1}    & 21.63                        & 22.21                        & \multicolumn{1}{c|}{19.49}    & 22.09                        & 22.32                        & \multicolumn{1}{c|}{20.57}       & 25.71                        & 26.73                        & 23.92                        \\
% \multicolumn{1}{l|}{-2}    & 23.85                        & \textbf{23.53}               & \multicolumn{1}{c|}{20.82}    & 24.04                        & \textbf{24.10}               & \multicolumn{1}{c|}{21.78}       & 26.05                        & \textbf{26.74}               & 24.77                        \\
% \multicolumn{1}{l|}{-3}    & \textbf{24.02}               & 23.14                        & \multicolumn{1}{c|}{24.38}    & \textbf{25}                  & 23.92                        & \multicolumn{1}{c|}{25.27}       & \textbf{27.03}               & 26.18                        & 28.2                         \\
% \multicolumn{1}{l|}{-4}    & 23.93                        & 23.05                        & \multicolumn{1}{c|}{25.80}    & 24.96                        & 23.88                        & \multicolumn{1}{c|}{\textbf{27}} & 26.59                        & 25.65                        & \textbf{29.64}               \\
% \multicolumn{1}{l|}{-5}    & 23.64                        & 17.23                        & \multicolumn{1}{c|}{oom}      & 24.77                        & 17.74                        & \multicolumn{1}{c|}{oom}         & 26.34                        & 20.09                        & oom                          \\
%                           & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         \\
%                           & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         \\
%                           & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}        
% \end{tabular}

% \end{table*}

% \begin{table}[]
% \footnotesize
% \centering
% \begin{tabular}{ccclc}
%       & \multicolumn{4}{c}{RefCOCO / RefCOCO+ / RefCOCOg}                             \\
% Layer & ViT-B/32              & ViT-B/16              & Layer & ViT-L/14              \\
% 12    & 21.63 / 22.09 / 25.71 & 22.21 / 22.32 / 26.73 & 24    & 19.49 / 20.57 / 23.92 \\
% 11    & 23.85 / 24.04 / 26.05 & 23.53 / 24.10 / 26.74 & 23    & 20.82 / 21.78 / 24.77 \\
% 10    & 24.02 / 25.00 / 27.03 & 23.14 / 23.92 / 26.18 & 22    & 24.38 / 25.27 / 28.20 \\
% 9     & 23.93 / 24.96 / 26.59 & 23.05 / 23.88 / 25.65 & 21    & 25.80 / 27.00 / 29.64 \\
% 8     & 23.64 / 24.77 / 26.34 & 17.23 / 17.74 / 20.09 & 20    & OOM / OOM /OOM       
% \end{tabular}
% \end{table}

\begin{table*}[]
\small
\centering
\label{tab:Token_masking}
\caption{The oIoU results with related to the masking layer and the model variants of CLIP. Global-context textual feature and mask proposals from FreeSOLO are used.}
\begin{tabular}{c|ccc|ccc|ccc}
\hline
                        & \multicolumn{3}{c|}{RefCOCO}                    & \multicolumn{3}{c|}{RefCOCO+}             & \multicolumn{3}{c}{RefCOCOg}                     \\ \hline
k                       & ViT-B/32       & ViT-B/16       & ViT-L/14      & ViT-B/32    & ViT-B/16      & ViT-L/14    & ViT-B/32       & ViT-B/16       & ViT-L/14       \\ \hline
1                       & 21.63          & 22.21          & 19.49         & 22.09       & 22.32         & 20.57       & 25.71          & 26.73          & 23.92          \\
2                       & 23.85          & \textbf{23.53} & 20.82         & 24.04       & \textbf{24.1} & 21.78       & 26.05          & \textbf{26.74} & 24.77          \\
3                       & \textbf{24.02} & 23.14          & 24.38         & \textbf{25} & 23.92         & 25.27       & \textbf{27.03} & 26.18          & 28.2           \\
4                       & 23.93          & 23.05          & \textbf{25.8} & 24.96       & 23.88         & \textbf{27} & 26.59          & 25.65          & \textbf{29.64} \\
5                       & 23.64          & 17.23          & -             & 24.77       & 17.74         & -           & 26.34          & 20.09          & -              \\
6                       & 23.54          & 15.71          & -             & 24.48       & 15.64         & -           & 25.97          & 16.89          & -              \\
7                       & 22.56          & 16.47          & -             & 23.6        & 17.1          & -           & 24.87          & 18.14          & -              \\
8                       & 22.01          & 16.02          & -             & 23.18       & 16.82         & -           & 24.15          & 17.63          & -              \\
9                       & 21.63          & 15.03          & -             & 22.81       & 15.63         & -           & 23.73          & 17.5           & -              \\
10                      & 21.23          & -              & -             & 22.33       & -             & -           & 23.5           & -              & -              \\
\multicolumn{1}{l|}{11} & 20.97          & -              & -             & 22.11       & -             & -           & 23.21          & -              & -              \\
\multicolumn{1}{l|}{12} & 20.59          & -              & -             & 21.71       & -             & -           & 23.05          & -              & -              \\ \hline
\end{tabular}
\end{table*}

==> tables/mask_feature_extractor.tex <==
% \begin{table}[]
% \caption{Experiments of different visual extractors on RefCOCO validation set. All method are based on CLIP and use only sentence as text feature. Grad-CAM and MaskCLIP don't use FreeSOLO. Hyperparameter k of Grad-CAM and Mask CLIP's score map is set to 0.1, 0.7.}
% \scriptsize{
% \centering
% \begin{tabular}{llccc}
% Methods                     & CLIP Model & RefCOCO & RefCOCO+ & RefCOCOg \\ \hline
% Grad-CAM(k=0.1)             & ResNet-50  & 10.74   & 10.85    & 10.64    \\
% MaskCLIP(k=0.7)             & ResNet-50  & 17.90   & 18.84    & 19.91    \\
% Adapting CLIP               & ViT-B/32   & 21.71   & 22.61    & 25.52    \\ \hline
% Local                    & ResNet-50  & 22.36   & 23.95    & 28.20    \\
% Global                    & ResNet-50  & 22.98   & 23.77    & 24.16    \\
% Global-Local             & ResNet-50  & 24.43   & 25.84    & 29.02    \\ \hline
% Local                   & ViT-B/32   & 22.73   & 24.09    & 28.69    \\
% Global                 & ViT-B/32   & 24.02   & 25.00    & 27.03    \\
% Global-Local             & ViT-B/32   & 24.85   & 26.14    & 30.18    \\ \hline
% Global                 & ViT-B/16   & 23.53   & 24.10    & 26.74    \\
% Global                 & ViT-L/14   & 25.80   & 27.00    & 29.64   
% \end{tabular}
% }
% \end{table}


\begin{table}[]
\caption{oIoU results of our method and two baselines including Grad-CAM and Dense score map where the mask can be predicted without FreeSOLO. Hyperparameter k of Grad-CAM and Dense score map is set to 0.1, 0.7.}
\scriptsize{
\centering
\begin{tabular}{llccc}
Methods                     & CLIP Model & RefCOCO & RefCOCO+ & RefCOCOg \\ \hline
Grad-CAM (k=0.1)             & ResNet-50  & 10.74   & 10.85    & 10.64    \\
Dense score map (k=0.7)     & ResNet-50  & 17.90   & 18.84    & 19.91    \\
Grad-CAM+FreeSOLO           & ResNet-50  & 14.02   & 14.46    & 12.51    \\
MaskCLIP+FreeSOLO           & ResNet-50  & 19.87   & 20.37    & 18.88    \\
Global-Local CLIP (Ours)    & ResNet-50  & 24.56   & 25.87    & 30.07   \\
\hline
\end{tabular}
}
\end{table}

==> tables/phrase_cut.tex <==
\begin{table}[]
\centering

\caption{Zero-shot evaluation with SoTA supervised methods on PhraseCut dataset. \textit{All} denotes the entire PhraseCut categories. \textit{Unseen} denotes a subset with classes not seen in RefCOCO.}
\label{tab:phrasecut}
\scalebox{0.7}{
\begin{tabular}{l|c|cc|cc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{Train dataset} & \multicolumn{2}{c|}{oIoU on val set}      & \multicolumn{2}{c}{oIoU on test set}      \\ \cline{3-6} 
\multicolumn{1}{c|}{}                        &                                & \multicolumn{1}{c}{All} & Unseen & \multicolumn{1}{c}{All} & Unseen \\ \hline
CRIS~\cite{cris}                              & RefCOCO                        & \multicolumn{1}{c}{16.43}    &    14.00    & \multicolumn{1}{c}{15.53}    &  13.75      \\ 
LAVT~\cite{lavt}                              & RefCOCO                        & \multicolumn{1}{c}{18.18}    &  15.26      & \multicolumn{1}{c}{16.68}    &   14.43     \\ \hdashline[1pt/1pt]
Ours (ViT-B/32)                         & N/A                            & \multicolumn{1}{c}{\textbf{22.91}}    &   \textbf{21.80}     & \multicolumn{1}{c}{\textbf{23.64}}    &   \textbf{22.98}     \\ \hline
\end{tabular}
}

\end{table}


==> tables/statistic_of_dataset.tex <==
\begin{table}[]
\footnotesize
\centering
\label{tab:statistic_dataset}
\caption{Statistics of datasets on the val split of RefCOCO, RefCOCO+ and RefCOCOg}
\begin{tabular}{c|ccc}
\hline
Category                 & RefCOCO & RefCOCO+ & RefCOCOg \\ \hline
Total number of sentence & 10834   & 10758    & 4896     \\ 
Average noun count       & 1.66    & 1.63     & 2.85     \\ 
Average word count       & 3.67    & 3.64     & 9.00     \\ \hline \hline
Textual features        & RefCOCO & RefCOCO+ & RefCOCOg \\ \cline{1-1}
Global-Local            & & & \\ 
Global                  & & & \\ \hline
\end{tabular}
\end{table}

==> tables/suple_NP_Sentence_same_ratio.tex <==
\begin{table}[h]
    \centering
    \small
    \caption{The ratio when the sentence is the target noun phrase on each datasets.}
    \begin{tabular}{l|ccc}
    \hline
         & RefCOCO & RefCOCO+ & RefCOCOg \\ \hline
    ratio &   0.4343 & 0.4861 & 0.0746 \\\hline
    \end{tabular}
    \label{tab:ratio_sen_np}
\end{table}

==> tables/suple_final_token_masking.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{\textcolor{blue}{[Results of our full model (global-local CLIP)] The final performance of global-context visual feature using optimal $k$ on each ViT variant. Global-context textual feature and mask proposals of FreeSOLO are used. We conduct the experiment on the val split of each dataset.}}
    \begin{tabular}{l|ccc}
    \hline
    ViT variants     & RefCOCO & RefCOCO+ & RefCOCOg  \\ \hline
    ViT-B/32     & 24.02 & 25.00 & 27.03 \\ 
    ViT-B/16 & 23.53 & 24.10 & 26.74 \\
    ViT-L/14 & 25.80 & 27.00 & 29.64 \\ \hline
    \end{tabular}
    \label{tab:final_token_masking}
\end{table}

==> tables/suple_global_local_textual.tex <==
\begin{table}[h]
\centering
\footnotesize
\caption{oIoU improvement of Global-Local textual feature on RefCOCO, RefCOCO+ and RefCOCOg validation set.}
\begin{tabular}{l|lll}
\hline
Textual feature    & RefCOCO & RefCOCO+ & RefCOCOg  \\ \hline
Global & 24.85 & 26.14 & 30.18 \\
Global-Local & 24.88(+0.3) & 26.16(+0.2) & 31.11(\textcolor{blue}{+0.93}) \\ \hline


\end{tabular}
\label{tab:oiou_results}
% \caption{123}
% \begin{tabular}{cc}
% \\
% 1     &1  \\
%  1    &1 
% \end{tabular}
\end{table}

